Online Velocity Profile Generation and Tracking for Sampling-Based Local Planning Algorithms in Autonomous Racing Environments

This work presents an online velocity planner for autonomous racing that adapts to changing dynamic constraints, such as grip variations from tire temperature changes and rubber accumulation. The method combines a forward-backward solver for online velocity optimization with a novel spatial sampling strategy for local trajectory planning, utilizing a three-dimensional track representation. The computed velocity profile serves as a reference for the local planner, ensuring adaptability to environmental and vehicle dynamics. We demonstrate the approach's robust performance and computational efficiency in racing scenarios and discuss its limitations, including sensitivity to deviations from the predefined racing line and high jerk characteristics of the velocity profile.

==> chapters/backup.tex <==
%%% ------------- PSEUDOCODE APEX DETECTION ---------------------

\begin{comment}
\begin{algorithm}[H]
\caption{This is a placeholder for the root finding algorithm which is unnecessarily long}
\label{alg:apex_determination}
\begin{algorithmic}[1]
\Require Offline raceline curvature at initial apex location $\Omega_z^\text{init}$
\Require Offline raceline velocity at initial apex $V_\text{init}$
\Require Interval around initial apex $[s_\text{min}, s_\text{max}]$
\Require Convergence tolerance $\epsilon$
\Require Maximum iterations $\text{max\_iter}$
\Require Scaling factor for feasible acceleration $\alpha$
\Ensure Feasible velocity at apex $V_\text{apex}$, Apex location $s_\text{apex}$
\State $V_\text{guess} \gets \sqrt{\alpha \cdot V_\text{init}}$ \Comment{Initial velocity estimate}
\State $V_\text{min} \gets \infty$ \Comment{Minimum velocity placeholder}
\State $s_\text{apex} \gets \text{None}$ \Comment{Apex location placeholder}

\For{$s \in [s_\text{min}, s_\text{max}]$} \Comment{Iterate over the interval}
    \State $V_\text{old} \gets V_\text{guess}$
    \For{$\text{iter} \gets 1, \text{max\_iter}$} \Comment{Fixed-point iteration}
        \State $a_y \gets \text{compute\_lateral\_acceleration}(s, V_\text{old})$
        \State $V_\text{new} \gets \sqrt{a_y / \Omega_z^\text{init}}$
        \If{$|V_\text{new} - V_\text{old}| < \epsilon$} \Comment{Check convergence}
            \State \textbf{break}
        \EndIf
        \State $V_\text{old} \gets V_\text{new}$
    \EndFor
    \If{$\text{iter} > \text{max\_iter}$} \Comment{Handle non-convergence}
        \State $V_\text{new} \gets V_\text{guess}$
    \EndIf
    \If{$V_\text{new} < V_\text{min}$}
        \State $V_\text{min} \gets V_\text{new}$
        \State $s_\text{apex} \gets s$
    \EndIf
\EndFor

\State $V_\text{apex} \gets V_\text{min}$\\
\Return $V_\text{apex}, s_\text{apex}$
\end{algorithmic}
\end{algorithm}
\end{comment}

% ------------------- SOTA BEHAVIORAL PLANNING ---------------------
Finally, behavioral planning governs high-level decision-making, such as complying with speed limits during a race or determining overtaking strategies \cite{sharma2021Recent}. In competitive autonomous racing, Chung et al. \cite{chung2025Autonomous} apply rendezvous guidance \cite{kunwar2006Motion} to assess whether an overtaking maneuver can be completed within a given time frame.
